Multiple Object Tracking with Mixture Density Networks for Trajectory Estimation

Multiple object tracking faces several challenges that may be alleviated with trajectory information. Knowing the posterior locations of an object helps disambiguating and solving situations such as occlusions, re-identification, and identity switching. In this work, we show that trajectory estimation can become a key factor for tracking, and present TrajE, a trajectory estimator based on recurrent mixture density networks, as a generic module that can be added to existing object trackers. To provide several trajectory hypotheses, our method uses beam search. Also, relying on the same estimated trajectory, we propose to reconstruct a track after an occlusion occurs. We integrate TrajE into two state of the art tracking algorithms, CenterTrack [63] and Tracktor [3]. Their respective performances in the MOTChallenge 2017 test set are boosted 6.3 and 0.3 points in MOTA score, and 1.8 and 3.1 in IDF1, setting a new state of the art for the CenterTrack+TrajE configuration

==> plots/bw_1/centertrack_gbs_OVERALL.tex <==
num bias MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 68.46 68.0 68.7 0.28 63.44 61.7 64.7 1.23 63.55 62.096 64.22 0.92 70.33 69.897 70.592 0.27 57.42 55.165 58.518 1.48
1 0.1 68.6 68.3 68.9 0.24 63.8 63.4 64.3 0.34 63.86 63.71 64.283 0.24 70.46 70.204 70.637 0.18 57.88 57.462 58.735 0.51
2 0.5 68.88 68.7 69.1 0.15 64.84 63.8 66.1 0.86 64.78 64.246 65.339 0.39 70.45 70.344 70.593 0.09 59.56 58.602 60.624 0.73
3 1 69.12 68.9 69.4 0.19 65.08 63.8 66.1 0.88 64.92 64.317 65.498 0.53 70.64 70.382 70.834 0.17 59.67 58.542 60.783 0.93
4 5 69.1 69.0 69.2 0.07 66.16 65.7 66.6 0.36 65.59 65.359 65.956 0.24 70.58 70.535 70.619 0.04 60.95 60.49 61.615 0.45
5 10 69.12 69.1 69.2 0.04 66.16 65.8 66.8 0.4 65.63 65.403 66.024 0.25 70.61 70.521 70.652 0.05 61.0 60.547 61.729 0.49

==> plots/bw_1/centertrack_pbs_OVERALL.tex <==
num bias MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 68.46 68.0 68.7 0.28 63.44 61.7 64.7 1.23 63.55 62.096 64.22 0.92 70.33 69.897 70.592 0.27 57.42 55.165 58.518 1.48
1 0.1 68.6 68.3 68.9 0.24 63.8 63.4 64.3 0.34 63.86 63.71 64.283 0.24 70.46 70.204 70.637 0.18 57.88 57.462 58.735 0.51
2 0.5 68.88 68.7 69.1 0.15 64.84 63.8 66.1 0.86 64.78 64.246 65.339 0.39 70.45 70.344 70.593 0.09 59.56 58.602 60.624 0.73
3 1 69.12 68.9 69.4 0.19 65.08 63.8 66.1 0.88 64.92 64.317 65.498 0.53 70.64 70.382 70.834 0.17 59.67 58.542 60.783 0.93
4 5 69.1 69.0 69.2 0.07 66.16 65.7 66.6 0.36 65.59 65.359 65.956 0.24 70.58 70.535 70.619 0.04 60.95 60.49 61.615 0.45
5 10 69.12 69.1 69.2 0.04 66.16 65.8 66.8 0.4 65.63 65.403 66.024 0.25 70.61 70.521 70.652 0.05 61.0 60.547 61.729 0.49

==> plots/bw_1/tracktor_gbs_OVERALL.tex <==
num bias seq MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 OVERALL 60.88 60.7 61.1 0.15 64.5 63.5 65.2 0.66 62.15 61.265 62.602 0.56 61.84 61.671 62.1 0.17 62.46 60.812 63.318 1.06
1 0.1 OVERALL 61.16 61.1 61.3 0.09 64.78 64.3 65.8 0.6 62.52 62.178 62.971 0.31 62.0 61.966 62.049 0.03 63.05 62.39 63.973 0.62
2 0.5 OVERALL 61.62 61.4 61.9 0.23 65.76 64.5 66.6 0.83 63.39 62.567 63.708 0.5 62.36 62.136 62.582 0.18 64.44 62.882 65.309 0.99
3 1 OVERALL 61.96 61.8 62.1 0.11 66.34 66.0 66.8 0.38 63.87 63.602 64.188 0.25 62.62 62.546 62.72 0.07 65.14 64.602 65.873 0.52
4 5 OVERALL 62.02 61.9 62.1 0.08 66.7 66.4 67.0 0.25 64.04 63.791 64.266 0.18 62.61 62.524 62.675 0.06 65.5 65.085 65.929 0.34
5 10 OVERALL 62.08 62.0 62.1 0.04 66.78 66.6 67.0 0.18 64.13 64.004 64.274 0.1 62.7 62.669 62.756 0.04 65.59 65.367 65.905 0.21

==> plots/bw_1/tracktor_pbs_OVERALL.tex <==
num bias seq MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 OVERALL 60.88 60.7 61.1 0.15 64.5 63.5 65.2 0.66 62.15 61.265 62.602 0.56 61.84 61.671 62.1 0.17 62.46 60.812 63.318 1.06
1 0.1 OVERALL 61.16 61.1 61.3 0.09 64.78 64.3 65.8 0.6 62.52 62.178 62.971 0.31 62.0 61.966 62.049 0.03 63.05 62.39 63.973 0.62
2 0.5 OVERALL 61.62 61.4 61.9 0.23 65.76 64.5 66.6 0.83 63.39 62.567 63.708 0.5 62.36 62.136 62.582 0.18 64.44 62.882 65.309 0.99
3 1 OVERALL 61.96 61.8 62.1 0.11 66.34 66.0 66.8 0.38 63.87 63.602 64.188 0.25 62.62 62.546 62.72 0.07 65.14 64.602 65.873 0.52
4 5 OVERALL 62.02 61.9 62.1 0.08 66.7 66.4 67.0 0.25 64.04 63.791 64.266 0.18 62.61 62.524 62.675 0.06 65.5 65.085 65.929 0.34
5 10 OVERALL 62.08 62.0 62.1 0.04 66.78 66.6 67.0 0.18 64.13 64.004 64.274 0.1 62.7 62.669 62.756 0.04 65.59 65.367 65.905 0.21

==> plots/bw_10/centertrack_gbs_OVERALL.tex <==
num bias MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 68.72 68.5 69.0 0.26 63.26 62.0 63.9 0.78 63.24 62.089 63.616 0.65 70.61 70.302 71.027 0.31 56.64 54.588 57.497 1.17
1 0.1 68.86 68.5 69.1 0.23 64.66 63.3 65.9 1.06 64.42 63.707 65.205 0.6 70.57 70.317 70.758 0.17 58.81 57.718 60.271 1.03
2 0.5 69.08 68.9 69.2 0.13 65.64 65.0 66.2 0.46 65.14 64.568 65.6 0.42 70.65 70.509 70.815 0.13 60.06 58.871 60.825 0.82
3 1 69.38 69.0 69.7 0.31 66.08 65.4 66.6 0.43 65.7 65.187 65.982 0.38 70.81 70.41 71.109 0.32 60.96 59.8 61.832 0.78
4 5 69.12 69.1 69.2 0.04 66.06 65.6 66.6 0.37 65.51 65.077 65.853 0.31 70.6 70.563 70.624 0.02 60.8 59.965 61.422 0.59
5 10 69.06 69.0 69.1 0.05 65.78 65.7 65.8 0.04 65.25 65.206 65.348 0.06 70.56 70.528 70.588 0.02 60.34 60.266 60.497 0.1

==> plots/bw_10/centertrack_pbs_OVERALL.tex <==
num bias MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 69.38 69.1 69.5 0.16 64.74 64.4 65.5 0.44 64.38 63.94 65.108 0.43 70.98 70.696 71.205 0.19 58.4 57.65 59.661 0.76
1 0.1 69.48 69.4 69.6 0.08 65.36 64.1 66.2 0.88 65.06 64.133 65.806 0.67 71.01 70.925 71.065 0.06 59.62 57.876 61.056 1.26
2 0.5 69.42 69.3 69.6 0.11 65.96 65.5 66.6 0.44 65.46 65.122 65.861 0.29 70.84 70.753 71.011 0.1 60.49 59.914 61.308 0.53
3 1 69.38 69.2 69.6 0.16 65.4 64.6 65.9 0.5 65.26 64.675 65.622 0.37 70.8 70.628 70.98 0.16 60.16 58.931 60.871 0.75
4 5 69.16 69.1 69.2 0.05 66.24 65.4 67.0 0.64 65.74 65.246 66.258 0.39 70.63 70.613 70.653 0.01 61.19 60.276 62.151 0.72
5 10 69.08 69.0 69.1 0.04 66.0 65.8 66.1 0.12 65.52 65.451 65.682 0.09 70.58 70.525 70.621 0.04 60.83 60.742 61.089 0.15

==> plots/bw_10/tracktor_gbs_OVERALL.tex <==
num bias seq MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 OVERALL 61.36 61.2 61.6 0.15 64.8 64.5 65.0 0.23 62.57 62.312 62.695 0.16 62.05 61.908 62.302 0.15 63.1 62.677 63.363 0.26
1 0.1 OVERALL 61.54 61.4 61.6 0.09 65.18 64.4 66.1 0.73 62.78 62.157 63.409 0.51 62.19 62.069 62.292 0.09 63.38 62.244 64.558 0.98
2 0.5 OVERALL 61.74 61.6 61.8 0.09 66.12 65.2 67.2 0.77 63.44 62.939 64.124 0.46 62.38 62.296 62.448 0.06 64.53 63.589 65.898 0.9
3 1 OVERALL 61.82 61.7 62.0 0.11 66.44 65.7 66.9 0.44 63.65 63.187 63.849 0.28 62.44 62.349 62.588 0.09 64.88 63.939 65.31 0.54
4 5 OVERALL 62.14 62.1 62.2 0.05 66.78 66.6 66.9 0.11 64.16 64.009 64.229 0.09 62.76 62.746 62.785 0.02 65.59 65.283 65.748 0.18
5 10 OVERALL 62.1 62.1 62.1 0.0 66.7 66.7 66.7 0.0 64.14 64.137 64.16 0.01 62.74 62.732 62.745 0.01 65.58 65.572 65.608 0.02

==> plots/bw_10/tracktor_pbs_OVERALL.tex <==
num bias seq MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 OVERALL 61.72 61.7 61.8 0.04 65.9 65.7 66.1 0.19 63.42 63.292 63.494 0.08 62.25 62.214 62.304 0.03 64.6 64.296 64.772 0.18
1 0.1 OVERALL 61.74 61.6 61.8 0.09 66.06 65.6 66.5 0.35 63.54 63.283 63.759 0.19 62.29 62.175 62.382 0.08 64.82 64.25 65.248 0.41
2 0.5 OVERALL 62.02 61.9 62.1 0.08 66.64 65.9 67.4 0.75 64.02 63.438 64.536 0.49 62.59 62.457 62.644 0.08 65.49 64.434 66.484 0.93
3 1 OVERALL 62.08 61.9 62.2 0.11 67.04 66.3 67.8 0.58 64.3 63.777 64.724 0.35 62.66 62.52 62.734 0.09 65.99 65.06 66.777 0.65
4 5 OVERALL 61.96 61.9 62.1 0.09 66.7 66.6 66.8 0.07 64.01 63.922 64.13 0.08 62.61 62.551 62.72 0.07 65.45 65.313 65.586 0.13
5 10 OVERALL 62.02 62.0 62.1 0.04 66.92 66.7 67.1 0.15 64.14 63.976 64.222 0.1 62.63 62.585 62.7 0.04 65.7 65.383 65.857 0.18

==> plots/bw_3/centertrack_gbs_OVERALL.tex <==
num bias MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 68.8 68.2 69.3 0.42 64.36 63.4 65.3 0.72 64.26 63.819 65.06 0.52 70.59 70.129 70.991 0.37 58.5 57.605 59.969 0.9
1 0.1 69.02 68.6 69.3 0.26 65.48 64.4 66.0 0.69 64.92 64.408 65.509 0.45 70.69 70.317 70.94 0.23 59.63 58.653 60.493 0.83
2 0.5 69.24 68.9 69.6 0.29 65.74 64.5 67.6 1.14 65.15 63.835 66.658 1.01 70.81 70.469 71.088 0.26 59.95 57.513 62.504 1.79
3 1 69.54 69.4 69.6 0.09 65.64 65.2 66.1 0.38 65.12 64.676 65.416 0.34 70.99 70.832 71.072 0.1 59.73 58.912 60.306 0.59
4 5 69.14 69.1 69.2 0.05 66.02 65.5 66.3 0.31 65.49 65.158 65.859 0.29 70.61 70.559 70.659 0.04 60.75 60.137 61.472 0.55
5 10 69.06 69.0 69.1 0.05 65.9 65.8 66.0 0.1 65.34 65.149 65.513 0.14 70.58 70.537 70.629 0.04 60.49 60.172 60.767 0.23

==> plots/bw_3/centertrack_pbs_OVERALL.tex <==
num bias MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 69.36 69.0 69.9 0.34 64.88 63.8 65.7 0.73 64.73 64.224 65.483 0.48 70.93 70.555 71.47 0.34 59.08 58.258 59.997 0.66
1 0.1 69.58 69.4 69.8 0.15 64.9 64.0 65.4 0.55 64.8 64.297 65.23 0.34 71.1 70.937 71.315 0.14 59.06 58.212 59.856 0.62
2 0.5 69.52 69.1 69.8 0.27 65.76 64.9 66.8 0.74 65.29 64.718 65.857 0.43 71.0 70.568 71.229 0.26 60.04 59.353 60.921 0.66
3 1 69.4 69.1 69.6 0.23 65.96 65.3 66.8 0.62 65.38 65.089 66.097 0.41 70.82 70.558 71.029 0.24 60.37 59.697 61.916 0.91
4 5 69.12 69.1 69.2 0.04 65.96 65.8 66.3 0.21 65.49 65.255 65.652 0.15 70.59 70.562 70.625 0.03 60.77 60.301 61.084 0.3
5 10 69.1 69.1 69.1 0.0 66.14 66.0 66.3 0.13 65.65 65.558 65.764 0.08 70.6 70.567 70.624 0.02 61.04 60.905 61.254 0.14

==> plots/bw_3/tracktor_gbs_OVERALL.tex <==
num bias seq MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 OVERALL 61.26 61.0 61.6 0.23 65.24 64.9 65.4 0.21 62.84 62.636 62.932 0.12 62.01 61.864 62.254 0.16 63.69 63.29 63.899 0.25
1 0.1 OVERALL 61.7 61.4 61.8 0.17 64.86 63.8 66.1 0.84 62.7 61.784 63.439 0.63 62.37 62.147 62.489 0.13 63.03 61.424 64.498 1.16
2 0.5 OVERALL 61.8 61.7 61.9 0.07 66.04 65.3 66.6 0.53 63.55 63.098 63.841 0.3 62.46 62.373 62.539 0.06 64.66 63.746 65.279 0.61
3 1 OVERALL 61.98 61.8 62.2 0.16 66.24 65.8 66.6 0.29 63.68 63.389 64.007 0.27 62.6 62.446 62.797 0.13 64.79 64.326 65.24 0.44
4 5 OVERALL 62.08 62.0 62.1 0.04 66.82 66.7 67.0 0.13 64.14 64.06 64.332 0.11 62.72 62.654 62.788 0.05 65.59 65.42 65.978 0.22
5 10 OVERALL 62.12 62.1 62.2 0.04 66.74 66.7 66.8 0.05 64.15 64.084 64.201 0.04 62.75 62.729 62.763 0.01 65.58 65.452 65.673 0.08

==> plots/bw_3/tracktor_pbs_OVERALL.tex <==
num bias seq MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 OVERALL 61.9 61.8 62.0 0.1 66.86 66.6 67.0 0.19 64.06 63.935 64.346 0.18 62.5 62.36 62.614 0.11 65.66 65.371 66.126 0.34
1 0.1 OVERALL 61.88 61.8 62.0 0.08 66.26 65.8 66.9 0.42 63.79 63.542 64.143 0.23 62.48 62.398 62.635 0.1 65.12 64.623 65.833 0.45
2 0.5 OVERALL 62.0 61.8 62.1 0.12 66.86 66.3 67.5 0.53 64.07 63.772 64.396 0.27 62.61 62.454 62.698 0.09 65.57 64.918 66.398 0.62
3 1 OVERALL 62.0 61.8 62.1 0.12 66.68 66.3 67.2 0.37 63.95 63.566 64.265 0.27 62.65 62.472 62.764 0.11 65.27 64.68 65.949 0.5
4 5 OVERALL 62.02 62.0 62.1 0.04 66.8 66.6 67.0 0.16 64.09 64.022 64.205 0.07 62.63 62.599 62.706 0.05 65.58 65.386 65.853 0.18
5 10 OVERALL 62.12 62.1 62.2 0.04 66.84 66.6 67.0 0.18 64.22 64.063 64.397 0.14 62.72 62.663 62.796 0.06 65.77 65.494 66.14 0.26

==> plots/bw_5/centertrack_gbs_OVERALL.tex <==
num bias MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 68.62 68.2 68.8 0.24 64.18 63.4 65.3 0.81 64.1 63.442 64.838 0.54 70.45 70.103 70.787 0.24 58.33 56.86 59.655 1.06
1 0.1 69.08 68.7 69.4 0.26 64.86 64.1 66.3 0.91 64.63 64.184 65.508 0.51 70.78 70.565 71.111 0.22 59.01 58.137 60.347 0.82
2 0.5 69.42 69.1 69.7 0.24 65.58 64.5 66.2 0.66 65.3 64.612 65.862 0.48 70.93 70.659 71.123 0.21 60.12 58.704 60.991 0.9
3 1 69.48 69.1 69.6 0.22 66.04 65.6 66.6 0.47 65.53 64.904 66.118 0.54 70.9 70.489 71.085 0.24 60.56 59.371 61.948 1.13
4 5 69.1 69.0 69.2 0.07 65.92 65.5 66.3 0.33 65.4 65.113 65.594 0.2 70.6 70.547 70.642 0.04 60.58 60.016 60.988 0.39
5 10 69.06 69.0 69.1 0.05 65.78 65.4 66.1 0.26 65.22 64.919 65.473 0.2 70.57 70.538 70.604 0.03 60.27 59.733 60.715 0.35

==> plots/bw_5/centertrack_pbs_OVERALL.tex <==
num bias MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 69.3 69.1 69.5 0.16 64.9 63.6 65.9 0.83 64.6 63.816 65.185 0.54 70.89 70.814 71.106 0.12 58.87 57.273 60.004 1.06
1 0.1 69.34 69.0 69.5 0.21 65.42 64.7 66.2 0.59 65.0 64.464 65.613 0.51 70.85 70.565 70.98 0.17 59.63 58.587 60.669 0.87
2 0.5 69.46 69.3 69.6 0.13 66.34 65.7 66.9 0.44 65.85 65.41 66.06 0.27 70.87 70.67 71.012 0.14 61.19 60.377 61.58 0.47
3 1 69.62 69.4 69.7 0.13 66.28 66.2 66.4 0.08 65.74 65.544 66.006 0.18 71.01 70.775 71.114 0.14 60.85 60.41 61.559 0.43
4 5 69.16 69.1 69.2 0.05 66.16 65.9 66.6 0.29 65.59 65.482 65.763 0.11 70.62 70.606 70.626 0.01 60.93 60.73 61.249 0.21
5 10 69.08 69.0 69.1 0.04 66.0 65.6 66.2 0.25 65.51 65.282 65.672 0.16 70.57 70.542 70.598 0.02 60.82 60.387 61.106 0.29

==> plots/bw_5/tracktor_gbs_OVERALL.tex <==
num bias seq MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 OVERALL 61.44 61.4 61.6 0.09 64.94 64.6 65.2 0.23 62.7 62.518 62.881 0.17 62.14 62.085 62.281 0.08 63.26 62.918 63.596 0.3
1 0.1 OVERALL 61.5 61.4 61.6 0.07 65.28 64.6 65.9 0.61 62.99 62.566 63.507 0.35 62.17 62.076 62.219 0.06 63.82 62.915 64.971 0.77
2 0.5 OVERALL 61.72 61.6 61.8 0.08 66.0 65.9 66.1 0.1 63.53 63.354 63.708 0.13 62.37 62.29 62.415 0.05 64.71 64.437 65.027 0.21
3 1 OVERALL 61.88 61.7 62.0 0.11 66.9 66.0 67.4 0.54 64.07 63.575 64.384 0.31 62.5 62.395 62.557 0.07 65.69 64.709 66.304 0.63
4 5 OVERALL 62.12 62.1 62.2 0.04 66.78 66.7 66.9 0.11 64.16 64.107 64.236 0.06 62.76 62.73 62.787 0.02 65.59 65.482 65.718 0.1
5 10 OVERALL 62.1 62.1 62.1 0.0 66.72 66.7 66.8 0.04 64.15 64.139 64.159 0.01 62.74 62.73 62.742 0.0 65.59 65.574 65.613 0.02

==> plots/bw_5/tracktor_pbs_OVERALL.tex <==
num bias seq MOTA_mean MOTA_min MOTA_max MOTA_std IDF1_mean IDF1_min IDF1_max IDF1_std HOTA_mean HOTA_min HOTA_max HOTA_std DetA_mean DetA_min DetA_max DetA_std AssA_mean AssA_min AssA_max AssA_std
0 0 OVERALL 61.78 61.7 61.9 0.11 66.66 66.3 66.9 0.23 63.91 63.493 64.186 0.28 62.34 62.258 62.448 0.1 65.51 64.746 66.066 0.53
1 0.1 OVERALL 62.04 61.9 62.3 0.17 66.54 66.2 66.9 0.25 63.88 63.591 64.315 0.28 62.59 62.438 62.826 0.16 65.2 64.366 65.989 0.6
2 0.5 OVERALL 62.02 61.9 62.2 0.11 66.9 66.1 67.7 0.62 64.14 63.578 64.7 0.43 62.6 62.456 62.785 0.12 65.72 64.72 66.673 0.77
3 1 OVERALL 62.04 61.9 62.1 0.09 67.04 66.6 67.6 0.43 64.18 63.798 64.595 0.29 62.61 62.534 62.652 0.05 65.78 65.034 66.598 0.59
4 5 OVERALL 62.0 61.9 62.1 0.07 66.98 66.6 67.4 0.3 64.21 63.908 64.446 0.2 62.63 62.541 62.758 0.08 65.82 65.219 66.326 0.42
5 10 OVERALL 62.06 61.9 62.1 0.09 66.86 66.7 67.2 0.23 64.16 64.116 64.265 0.06 62.66 62.552 62.729 0.07 65.69 65.577 65.918 0.14

==> tables/ablation_2.tex <==
\begin{table}
\center
\tabcolsep=0.11cm

     \resizebox{\columnwidth}{!}{
    \begin{tabular}{l l c c c c c c c }\\
     \toprule
     Sequence & Method & MOTA $\uparrow$ & IDF1 $\uparrow$ & MT $\uparrow$ & ML $\downarrow$ & FP $\downarrow$ & FN $\downarrow$ & ID Sw. $\downarrow$ \\ [0.5ex] 
 MOT17-02 & Greedy search & 43.8 & 52.0 & 10 & 22 & 80  & 10337 & 32  \\
 MOT17-02 & Pure beam search & 45.2 & 52.9 & 14 & 22 & 254  & 9905 & 32  \\
  MOT17-04 & Greedy search & 64.7 & 74.0 & 35 & 22 & 80  & 16675 & 11  \\
  MOT17-04 & Pure beam search  & 64.8 & 75.4 & 35 & 22 & 130  & 16597 & 11  \\
  MOT17-05 & Greedy search & 56.6 & 64.5 & 36 & 35 & 165 & 2791  & 43  \\
  MOT17-05 & Pure beam search  & 51.0 & 57.1 & 36 & 35 & 681 & 2664  & 42  \\
  MOT17-10 & Greedy search & 69.1 & 57.3 & 25 & 2  & 241 & 3574  & 147 \\
  MOT17-10 & Pure beam search  & 69.1 & 57.3 & 25 & 2  & 241 & 3574  & 147 \\
  
      \end{tabular}}
\vspace{0.2mm}
\caption{Ablation studio on both greedy and pure beam search methods. }
\label{tab:ablation1}

\end{table}

==> tables/ablation_beam.tex <==
\begin{table}
\center
\tabcolsep=0.11cm
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c c c c c c c c c }\\
         \toprule
     Beam width & MOTA $\uparrow$ & IDF1 $\uparrow$ & MT $\uparrow$ & ML $\downarrow$ & FP $\downarrow$ & FN $\downarrow$ & ID Sw. $\downarrow$ & Hz. $\uparrow$ \\ [0.5ex] 
     \midrule
    1 & 61.7 & 66.5 & 198 & 111 & 1323 & 41189 & 459    & 3   \\
    2 & 61.7 & 66.5 & 198 & 111 & 1291 & 41259 & 470    & 2.4 \\
    5 & 62.2 & 66.9 & 237 & 110 & 875  & 41127 & 434    & 1.3 \\
    10 & 62.0 & 67.4 & 199 & 110 & 997  & 41257 & 452    & 0.5    
     \midrule
    \end{tabular}}
\vspace{0.5mm}
\caption{Ablation studio on the beam search width $B$. We evaluate on the Faster R-CNN of MOT17 public detections.}
\label{tab:ablation1}

\end{table}


==> tables/mot_1617.tex <==
\begin{table}
\center
\tabcolsep=0.11cm

    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l c c c c c c c }
     \toprule
     Method & MOTA $\uparrow$ & IDF1 $\uparrow$ & MT \% $\uparrow$ & ML \% $\downarrow$ & FP $\downarrow & FN $\downarrow & ID Sw. $\downarrow$ \\ [0.5ex] 
     \midrule

     \multicolumn{8}{c}{MOT16~\cite{MOT16} \vspace{1mm}} \\
     \midrule
     % 67.76	78.34	61.39	71.19	53.97	72.09	95.09	406760	20982	157468	36.01	39.45	24.54	848	929	578	1.18	5668	78.62	3475	48.2
    
     Ours (Tracktor + TrajE) &  \color{red}\textbf{56.1} & \color{red}\textbf{56.9} & \color{red}\textbf{21.5} &  \color{blue}\textit{35.4} & \color{blue}\textit{3691} & \color{red}\textbf{75628} &  742  \\
     Tracktor \cite{bergmann2019tracking} & \color{blue}\textit{54.4} &  52.5  & 19.0 & 36.9 &  \color{red}\textbf{3280} & \color{blue}\textit{79149} & 682 \\
     NOTA \cite{chen2019aggregate}  & 49.8 & 55.3 &	17.9 & 37.7 & 7428 & 83614 & 614 \\
     HCC \cite{ma2018customized}  & 49.3 & 50.7 & 17.8 & 39.9 & 5333 & 86795 & \color{red}\textbf{391} \\
     ETC \cite{wang2019exploit} & 49.2 & \color{blue}\textit{56.1} & 17.3 & 40.3 & 8400 & 83702 & 882 \\  
     AFN \cite{shen2018tracklet} & 49.0 & 48.2 &	\color{blue}\textit{19.1} & 35.7 & 9508 & 82506 & 1383 \\
     LMP \cite{tang2017multiple} & 48.8 & 51.3 & 18.2 & 40.1 & 6654 & 86245 & \color{blue}\textit{481} \\
     KCF \cite{chu2019online}  & 48.8 & 47.2 & 15.8 & 38.1 & 5875 & 86567 & 906 \\
     STRN \cite{xu2019spatial} & 48.5 & 53.9 & 17.0 & \color{red}\textbf{34.9} & 9038 & 84178 & 747 \\
     GCRA \cite{ma2018trajectory} & 48.2 & 48.6 & 12.9 & 41.1 & 5104 & 88586 & 821 \\
     FWT \cite{henschel2017improvements}  & 47.8 & 44.3 & \color{blue}\textit{19.1} & 38.2 & 8886 & 85487 & 852 \\
     \\
     \midrule
     \multicolumn{8}{c}{ MOT17~\cite{MOT16} \vspace{1mm}  } \\
     \midrule
     % MOTA IDF1 MT	ML	FP	FN	 Sw.	
     \textbf{Ours} (CenterTrack + TrajE) &  \color{red}\textbf{67.8} & \color{red}\textbf{61.4} & \color{red}\textbf{36.0} &  \color{red}\textbf{24.5} & 20982 & \color{red}\textbf{157468} &  3475  \\
     
     CenterTrack \cite{zhou2020tracking} & \color{blue}\textit{61.5} & \color{blue}\textit{59.6} & \color{blue}\textit{26.4} &  \color{blue}\textit{31.9} & 14076 & \color{blue}\textit{200672} & 2583 \\
     
     Lif\_T \cite{hornakova2020lifted}  & 60.5 & 65.6 & 27.0 & 33.6 & 14966  & 206619 & 1189 \\
     MPNTrack \cite{braso2020learning} & 58.8 & 61.7 & 28.8 & 33.5 & 17413 & 213594 & 1185 \\
     
     \textbf{Ours} (Tracktor(v2) + TrajE) & 56.6 & 58.2 & 21.9 & 35.7 & 10119 & 231091 & 2442 \\
     Tracktor(v2)\cite{bergmann2019tracking} & 56.3 & 55.1 & 21.1 & 35.3 & \color{red}\textbf{8866} & 235449 & 1987 \\
     
     \textbf{Ours} (Tracktor++) + TrajE) & 56.0 & 57.2 & 22.6 & 35.1 & 14378 & 231212 & 2546 \\
     
     TT17   \cite{zhang2020long}  & 54.9 & 63.1 & 24.4 & 38.1 & 20236 & 233295 & 1088  \\
     TPM    \cite{peng2020tpm}  & 54.2 & 52.6 & 22.8 & 37.5 & 13739 & 242730 & 1824 \\
     
     Tracktor++\cite{bergmann2019tracking} & 53.5 & 52.3 & 19.5 & 36.6 & \color{blue}\textit{12201} & 248047 & 2072 \\
     JBNOT \cite{henschel2019multiple} & 52.6 & 50.8 & 19.7 & 35.8 & 31572 & 232659 & 3050 \\
     FAMNet \cite{chu2019famnet} & 52.0 & 48.7 & 19.1 & 33.4 & 14138 & 253616 & 3072 \\   
     ETC \cite{wang2019exploit} & 51.9 & 58.1 & 23.1 & 35.5 & 36164 & 232783 & 3071 \\   
     eHAF\cite{sheng2018heterogeneous} & 51.8 & 54.7 & 23.4 & 37.9 & 33212 & 236772 & \color{blue}\textit{1834} \\
     AFN \cite{shen2018tracklet} & 51.5 &	46.9 &	20.6 & 35.5 & 22391 & 248420 & 2593 \\
     NOTA \cite{chen2019aggregate} & 51.3 &	54.7 &	17.1 & 35.4 & 20148 & 252531 & 2285 \\
     FWT \cite{henschel2017improvements} & 51.3 & 47.6 & 21.4 & 35.2 & 24101 & 247921 & 2648 \\
     jCC \cite{keuper2018motion} & 51.2 & 54.5   & 20.9 & 37.0 & 25937 & 247822 & \color{red}\textbf{1802}\\
     STRN \cite{xu2019spatial} & 50.9 & 56.0 & 18.9 & 33.8 & 25295 & 249365 & 2397 \\

     \bottomrule
    \end{tabular}}
\vspace{0.1cm}
\caption{Comparison integrating \textit{TrajE} to CenterTrack and Tracktor (version 1 and 2) with state-of-the art methods on the MOTChallenge dataset for both 2016 and 2017 versions using public detections. }
\vspace{-0.2cm}
\label{tab:mot}

\end{table}

==> tables/mot_old.tex <==
\begin{table}
\center
\tabcolsep=0.07cm

    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l c c c c c c c }
     \midrule
     \multicolumn{8}{c}{ MOT17~\cite{MOT16} \vspace{1mm}  } \\
     \toprule
     Method & MOTA $\uparrow$ & IDF1 $\uparrow$ & MT \% $\uparrow$ & ML \% $\downarrow$ & FP $\downarrow & FN $\downarrow & ID Sw. $\downarrow$ \\ [0.5ex] 
     \midrule
     % MOTA IDF1 MT	ML	FP	FN	 Sw.	
     \textbf{Ours} (CenterTrack + TrajE) &  \color{red}\textbf{67.8} & \color{red}\textbf{61.4} & \color{red}\textbf{36.0} &  \color{red}\textbf{24.5} & 20982 & \color{red}\textbf{157468} &  3475  \\
     
     CenterTrack \cite{zhou2020tracking} & \color{blue}\textit{61.5} & \color{blue}\textit{59.6} & \color{blue}\textit{26.4} &  \color{blue}\textit{31.9} & 14076 & \color{blue}\textit{200672} & 2583 \\
     
     Lif\_T \cite{hornakova2020lifted}  & 60.5 & 65.6 & 27.0 & 33.6 & 14966  & 206619 & 1189 \\
     MPNTrack \cite{braso2020learning} & 58.8 & 61.7 & 28.8 & 33.5 & 17413 & 213594 & 1185 \\
     
     \textbf{Ours} (Tracktor(v2) + TrajE) & 56.6 & 58.2 & 21.9 & 35.7 & 10119 & 231091 & 2442 \\
     Tracktor(v2)\cite{bergmann2019tracking} & 56.3 & 55.1 & 21.1 & 35.3 & \color{red}\textbf{8866} & 235449 & 1987 \\
     
     \textbf{Ours} (Tracktor++) + TrajE) & 56.0 & 57.2 & 22.6 & 35.1 & 14378 & 231212 & 2546 \\
     
     TT17   \cite{zhang2020long}  & 54.9 & 63.1 & 24.4 & 38.1 & 20236 & 233295 & 1088  \\
     TPM    \cite{peng2020tpm}  & 54.2 & 52.6 & 22.8 & 37.5 & 13739 & 242730 & 1824 \\
     
     Tracktor++\cite{bergmann2019tracking} & 53.5 & 52.3 & 19.5 & 36.6 & \color{blue}\textit{12201} & 248047 & 2072 \\
     JBNOT \cite{henschel2019multiple} & 52.6 & 50.8 & 19.7 & 35.8 & 31572 & 232659 & 3050 \\
     FAMNet \cite{chu2019famnet} & 52.0 & 48.7 & 19.1 & 33.4 & 14138 & 253616 & 3072 \\   
     ETC \cite{wang2019exploit} & 51.9 & 58.1 & 23.1 & 35.5 & 36164 & 232783 & 3071 \\   
     eHAF\cite{sheng2018heterogeneous} & 51.8 & 54.7 & 23.4 & 37.9 & 33212 & 236772 & \color{blue}\textit{1834} \\
     AFN \cite{shen2018tracklet} & 51.5 &	46.9 &	20.6 & 35.5 & 22391 & 248420 & 2593 \\
     NOTA \cite{chen2019aggregate} & 51.3 &	54.7 &	17.1 & 35.4 & 20148 & 252531 & 2285 \\
     FWT \cite{henschel2017improvements} & 51.3 & 47.6 & 21.4 & 35.2 & 24101 & 247921 & 2648 \\
     jCC \cite{keuper2018motion} & 51.2 & 54.5   & 20.9 & 37.0 & 25937 & 247822 & \color{red}\textbf{1802}\\
     STRN \cite{xu2019spatial} & 50.9 & 56.0 & 18.9 & 33.8 & 25295 & 249365 & 2397 \\

     \bottomrule
    \end{tabular}}
\vspace{0.1cm}
\caption{Comparison integrating \textit{TrajE} to CenterTrack and Tracktor (version 1 and 2) with state-of-the art methods on the MOTChallenge 17 dataset using public detections.}
\vspace{-0.2cm}
\label{tab:mot17}

\end{table}

==> tables/phd_def.tex <==
\begin{table}[t!]
\center
\tabcolsep=0.07cm

    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l c c c c c c }
     \toprule
     \multicolumn{7}{c}{ MOT17~ \vspace{1mm}  } \\
     \midrule
     Method & MOTA $\uparrow$ & IDF1 $\uparrow$ & MT \% $\uparrow$ & ML \% $\downarrow$ & FP $\downarrow & FN $\downarrow \\ [0.5ex] 
     \midrule
     CenterTrack & {61.5} & 59.6 & 26.4 &  {31.9} & 14076 & {200672}\\
     {+TrajE} &  {67.4}(+5.9) & {61.2}(+1.6) & {34.8} &  {24.9} & 18652 & {161347}  \\
     {+TrajE+occ} &  {67.8}(+6.3) & 61.4(+1.8) & {36.0} &  {24.5} & 20982 & {157468}  \\
     \midrule
     Tracktor & 56.3 & 55.1 & 21.1 & 35.3 & {8866} & 235449 \\
     {+TrajE} & 56.3(+0.0) & 57.8(+2.7) & 21.4 & 35.8 & {10068} & 233885  \\
     
     {+TrajE+occ} & 56.6(+0.3) & 58.2(+3.1) & 21.9 & 35.7 & {10119} & 231091  \\
     
     \bottomrule
    \end{tabular}}
\vspace{0.05cm}
\caption{Comparison integrating \textit{TrajE} to CenterTrack and Tracktor against the state of the art methods on the test set of MOTChallenge 17 dataset using public detections. In bold tracker + our method (TrajE). In red the best result, in blue the second best. The tracking baselines are CenterTrack+OFF, Tracktor+CV+CMC.}
\label{tab:mot17}
\vspace{-1mm}
\end{table}

==> tables/phd_def_ua.tex <==
\begin{table}[t!]
\center
\tabcolsep=0.07cm

    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l c c c c c c }
     \toprule
     \multicolumn{7}{c}{ UA-DETRAC~ \vspace{1mm}  } \\
     \midrule
     Method & MOTA $\uparrow$ & IDF1 $\uparrow$ & MT \% $\uparrow$ & ML \% $\downarrow$ & FP $\downarrow & FN $\downarrow \\ [0.5ex] 
     \midrule
     CenterTrack & {61.5} & 59.6 & 26.4 &  {31.9} & 14076 & {200672}\\
     {+TrajE} &  {67.4}(+5.9) & {61.2}(+1.6) & {34.8} &  {24.9} & 18652 & {161347}  \\
     {+TrajE+occ} &  {67.8}(+6.3) & 61.4(+1.8) & {36.0} &  {24.5} & 20982 & {157468}  \\
     \midrule
     Tracktor & 56.3 & 55.1 & 21.1 & 35.3 & {8866} & 235449 \\
     {+TrajE} & 56.3(+0.0) & 57.8(+2.7) & 21.4 & 35.8 & {10068} & 233885  \\
     
     {+TrajE+occ} & 56.6(+0.3) & 58.2(+3.1) & 21.9 & 35.7 & {10119} & 231091  \\
     
         \textbf{CenterTrack + TrajE} & \color{red}\textbf{72.0} & \color{red}\textbf{80.8} & \color{red}\textbf{72.5} & 7.4 & 44415 & \color{red}\textbf{130911}  \\
    CenterTrack \cite{zhou2020tracking} & \color{blue}{69.9} & \color{blue}{78.1} & \color{blue}{71.5} & 8.5 & 46657 & \color{blue}{141356} \\
     
    \textbf{Tracktor(v2) + TrajE} & 69.2 & 76.1 & 62.2 & 9.3 & \color{blue}{26236} & 181029 \\
     
     \bottomrule
    \end{tabular}}
\vspace{0.05cm}
\caption{Comparison integrating \textit{TrajE} to CenterTrack and Tracktor against the state of the art methods on the test set of MOTChallenge 17 dataset using public detections. In bold tracker + our method (TrajE). In red the best result, in blue the second best. The tracking baselines are CenterTrack+OFF, Tracktor+CV+CMC.}
\label{tab:mot17}
\vspace{-1mm}
\end{table}

==> tables/ua-detrac_old.tex <==
\begin{table}
\center
\tabcolsep=0.11cm

    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l c c c c c c}
     \toprule
     \multicolumn{7}{c}{UA-DETRAC~\cite{CVIU_UA-DETRAC} \vspace{1mm}} \\
     \midrule
     Method & MOTA $\uparrow$ & MT \% $\uparrow$ & ML \% $\downarrow$ & MOTP $\uparrow$ & FP $\downarrow$ & FN $\downarrow$  \\ [0.5ex] 
     \midrule
     % 67.76	78.34	61.39	71.19	53.97	72.09	95.09	406760	20982	157468	36.01	39.45	24.54	848	929	578	1.18	5668	78.62	3475	48.2
    
    Ours (CenterTrack + TrajE) & 65.8 & 69.9 & 6.3 & 83.2 & 88517 & 132870  \\
    CenterTrack \cite{zhou2020tracking} & - & - & - & - & - & - \\
    Ours (Tracktor v2 + TrajE) & 69.2 & 62.2 & 9.3 & 82.5 & 26236 & 181029 \\
    Tracktor v2 \cite{bergmann2019tracking} & 67.7 & 60.0 & 9.9 & 82.6 & 23422 & 193526\\
    WD \cite{zeng2020robust} & 68.5 & 70.2 & 3.1 & 86.5 & - & -\\
    DeepSORT \cite{wojke2017simple} & 65.4 & 65.9 & 4.7 & 86.3 & - & -\\
    POI \cite{yu2016poi} & 69.2 & 67.4 & 5.2 & 86.1 & - & -\\
    RMOT \cite{yoon2015bayesian} & 62.6 & 42.1 & 6.5 & 75.7 & - & -\\
    IHTLS \cite{dicle2013way} & 62.6 & 63.4 & 3.8 & 82.2 & - & - \\
    
    \bottomrule
    \end{tabular}}
\vspace{0.1cm}
\caption{Comparison integrating \textit{TrajE} to CenterTrack and Tracktor with state-of-the art methods on the UA-DETRAC dataset using CompACT \cite{cai2015learning} public detections.}
\vspace{-0.2cm}
\label{tab:ua-detrac}

\end{table}




==> tables/vot_table.tex <==
\begin{table}[t]

\centering
\caption{Performance comparisons on public short-term benchmarks. OP: mean overlap precision at the threshold of 0.5; DP: mean distance precision of 20 pixels; EAO: expected average overlap, and mean speed (FPS). The {\color{red}\textbf{red bold}} fonts and {\color{blue}\textit{blue italic}} fonts indicate the best and the second best performance.}
\label{tab:component}
\begin{tabular}{|c|cc|ccc|ccc|ccc|c|}
\hline
\multirow{2}{*}{Trackers} & \multicolumn{2}{c|}{OTB-2015} & \multicolumn{3}{c|}{VOT2015} & \multicolumn{3}{c|}{VOT2016} & \multicolumn{3}{c|}{VOT2017} & \multicolumn{1}{c|}{\multirow{2}{*}{FPS}} \TBstrut\\
\cline{2-12} & OP & DP & A & R & EAO & A & R & EAO & A & R & EAO&  \Tstrut\\ \hline\hline
SiamFC  & 73.0 & 77.0 & 0.533 & 0.88 & 0.289 & 0.53 & 0.46 & 0.235 & 0.50 & 0.59 & 0.188 & 86\Tstrut\\
CFNet   & 69.9 & 74.7 & - & - & - & - & - & - & - & - & - & 75\Tstrut\\
Staple  & 70.9 & 78.4 & 0.57 & 1.39 & 0.300 & 0.54 & 0.38 & 0.295 & \color{blue}\textit{0.52} & 0.69 & 0.169 & 80\Tstrut\\
CSRDCF  & 70.7 & 78.7 & 0.56 & 0.86 & 0.320 & 0.51 & 0.24 & 0.338 & 0.49 & 0.36 & 0.256 & 13\Tstrut\\
%PTAV   & 81.2 & 87.9 & 76.8 & 84.1 & - & - & - & - & - & - & - & - & - & 15\Tstrut\\
BACF    & 76.7 & 81.5 & 0.59 & 1.56 & - & - & - & - & - & - & - & 35\Tstrut\\
ECO-HC  & 78.4 & 85.6 & - & - & - & 0.54 & 0.30 & 0.322 & 0.49 & 0.44 & 0.238 & 60\Tstrut\\
\hline\hline
%SINT  & 81.6 & 88.1 & 71.9 & 78.8 & - & - & - & - & - & - & - & - & - & 5\Tstrut\\
CREST  & 77.5 & 83.7 & - & - & - & 0.51 & 0.25 & 0.283 & - & - & - & 1\Tstrut\\
MDNet  & \color{blue}\textit{85.4} & \color{blue}\textit{90.9} & \color{blue}\textit{0.60} & \color{blue}\textit{0.69} & \color{blue}\textit{0.378} & 0.54 & 0.34 & 0.257 & - & - & - & 1\Tstrut\\
C-COT  & 82.0 & 89.8 & 0.54 & 0.82 & 0.303 & 0.54 & 0.24 & 0.331 & 0.49 & \color{blue}\textit{0.32} & 0.267 & 0.3\Tstrut\\
ECO    & 84.9 & \color{red}\textbf{91.0} & - & - & - & 0.55 & \color{red}\textbf{0.20} & \color{blue}\textit{0.375} & 0.48 & \color{red}\textbf{0.27} & \color{blue}\textit{0.280} & 8\Tstrut\\
\hline\hline
SiamRPN    & 81.9 & 85.0 & 0.58 & 1.13 & 0.349 & \color{blue}\textit{0.56} & 0.26 & 0.344 & 0.49 & 0.46 & 0.244 & {\color{red}\textbf{200}}\Tstrut\\
\textbf{Ours} & {\color{red}\textbf{86.5}} & 88.0 & \color{red}\textbf{0.63} & \color{red}\textbf{0.66} & \color{red}\textbf{0.446} & \color{red}\textbf{0.61} & \color{blue}\textit{0.22} & \color{red}\textbf{0.411} & \color{red}\textbf{0.56} & 0.34 & \color{red}\textbf{0.326} & {\color{blue}\textit{160}}\Tstrut\\
\hline
\end{tabular}

\end{table}
